Automata and Graph Compression

We present a theoretical framework for the compression of automata, which are widely used in speech processing and other natural language processing tasks. The framework extends to graph compression. Similar to stationary ergodic processes, we formulate a probabilistic process of graph and automata generation that captures real world phenomena and provide a universal compression scheme LZA for this probabilistic model. Further, we show that LZA significantly outperforms other compression techniques such as gzip and the UNIX compress command for several synthetic and real data sets.

==> comments.tex <==
%2) Q* contains the empty set (and anyway X \cup {{}} was the right version) - removed latter. Change notaton to \phi inther uses.

%3) isomorphic automaton not defined in first use.

%4) changed 'models on automata' to 'models of automata'

%7) difference encoding talks about 'vertices' - not 'nodes' or 'states'.

8) LZA section refers to non-empty transitions and non-zero labeled transitions. Neither makes sense in the current notation. 

9) 'transition label' function is odd terminology (at least to me). It is a 'transition function' that maps from a state and label to destination states.
Terminology should reflect that. I changed first use, but there are numerous others that need to be fixed.

Maybe you should mention how you want to deal with this first just to get a nice notation. Looks to me like you still have the notation from when
you were considering more restricted automata. Anyway, it is in a lot of places.


%11) "There are several probabilistic models of automata and graphs that satisfy this property."  Say which property and why it is relevant in th non-sequence case.

%2) Q* contains the empty set (and anyway X \cup {{}} was the right version) - removed latter. Change notaton to \phi inther uses.

%I meant 'Changed notation ....' 

%Fix the last two theorems

%2. Change algorithm into algorithm environment



